BiomedJourney: Counterfactual Biomedical Image Generation by Instruction-Learning from Multimodal Patient Journeys

Rapid progress has been made in instruction-learning for image editing with natural-language instruction, as exemplified by InstructPix2Pix. In biomedicine, such methods can be applied to counterfactual image generation, which helps differentiate causal structure from spurious correlation and facilitate robust image interpretation for disease progression modeling. However, generic image-editing models are ill-suited for the biomedical domain, and counterfactual biomedical image generation is largely underexplored. In this paper, we present BiomedJourney, a novel method for counterfactual biomedical image generation by instruction-learning from multimodal patient journeys. Given a patient with two biomedical images taken at different time points, we use GPT-4 to process the corresponding imaging reports and generate a natural language description of disease progression. The resulting triples (prior image, progression description, new image) are then used to train a latent diffusion model for counterfactual biomedical image generation. Given the relative scarcity of image time series data, we introduce a two-stage curriculum that first pretrains the denoising network using the much more abundant single image-report pairs (with dummy prior image), and then continues training using the counterfactual triples. Experiments using the standard MIMIC-CXR dataset demonstrate the promise of our method. In a comprehensive battery of tests on counterfactual medical image generation, BiomedJourney substantially outperforms prior state-of-the-art methods in instruction image editing and medical image generation such as InstructPix2Pix and RoentGen. To facilitate future study in counterfactual medical generation, we plan to release our instruction-learning code and pretrained models.

==> figs/attention_heatmap/prompts.tex <==
right large pleural effusion
severe cardiomegaly

==> figs/example_fig/prompts.tex <==
% id
p19/p19932242/s52061976/56c9c87c-841a4a08-8bab7f02-e3b8ffd7-62fff702
% source impression
_ year old man with myeloma , cough // Pneumonia As compared to the previous examination , there is a newly developed middle lobe pneumonia . The pneumonia is ill - defined an shows multiple air bronchograms . Otherwise the lung parenchyma is unremarkable . Normal size of the cardiac silhouette . No pleural effusions . At the time of dictation and observation , the referring physician was paged , _ , 13:23 . Findings were discussed _ min later over the telephone .
% target impression
Resolving right middle lobe pneumonia. A followup chest radiograph in 4 weeks is recommended. If the right middle lobe opacity fails to completely resolve by that time, a chest CT should be performed at that time to exclude an endobronchial lesion. New small right pleural effusion.
% gpt4 impression
Resolving right middle lobe pneumonia. New small right pleural effusion.
% gpt4 generated disease progression
Newly developed middle lobe pneumonia with air bronchograms, new small right pleural effusion, and accessed right pectoral MediPort extends to superior cavoatrial junction.

==> figs/model_comparison/prompt.tex <==
% id
p19/p19630335/s52550136/e65e6068-cc8ab4e2-f829f4ce-7a1aefa4-98f3700e
% impression
In comparison with the study _ _, there again are low lung volumes. There is and increasing right pleural effusion with increased prominence of the cardiac silhouette. No evidence of pleural effusion on the left. Increased prominence of central pulmonary vessels, though no evidence of peripheral venous congestion.
% gpt4
There is an increasing right pleural effusion with increased prominence of the cardiac silhouette. No evidence of left pleural effusion. Increased prominence of central pulmonary vessels is observed, with no evidence of peripheral venous congestion.

==> figs/segmentation_model_comparison/meta.tex <==
\begin{table}
    \centering
    \begin{tabular}{ccccccc}
         &  gold&  real img&  sd&  ip2p&  roetgen& medjourney
\\
         race&  white&  white&  white&  black&  white& white
\\
         age&  50&  57.82&  51.6&  40.21&  73.82& 54.03
\\
         gender&  M&  &  &  &  F& \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> texts/method-backup.tex <==
\section{Method}

\subsection{Problem Definition}

Given the prior image $\textbf{I}_P \in \mathcal{R}^{H \times W \times 3}$ and a progression description $\textbf{D}$, the goal of counterfactual medical image generation is to learn a generative model $Gen$ for generating the counterfactual image $\textbf{I}_C \in \mathcal{R}^{H \times W \times 3}$, \textit{i.e.}, $\textbf{I}_C = Gen(\textbf{I}_P, \textbf{D})$.

Compared to text-only medical image generation models such as RoentGen~\citep{chambon2022roentgen}, our problem setting is very different: the generation description $\textbf{D}$ describes the counterfactual changes from the prior image to the target image, rather than the description of the target image itself. This means that the model inputs both textual description and the prior image and is expected to produce a new image that reflects the prescribed changes while preserving other invariant aspects in the prior image. %These unique challenges necessitate new model design, training, and evaluation strategies, which we elaborate below.

%but differs in three aspects: $(i)$ the instruction $\textbf{P}$ is supposed to describe the temporal changes from source to target image, rather than the target image itself; $(ii)$ the model takes both textual instruction and source image as its inputs; $(iii)$ the model is expected to make desired content modifications while preserving remaining components in the source image. These unique challenges necessitate a new model design, training, and evaluation strategies, which we elaborate below.

\subsection{\ourmodel{}}
\label{Sec:Medjourney}

We build upon the state-of-the-art latent diffusion model (LDM)~\citep{rombach2022highresolution}, which comprises two components: 
\begin{itemize}[leftmargin=*]
    \item An image autoencoder based on VQGAN that can project an image to $z$ in latent space and then reconstruct the image from $z$.
    \item A UNet~\cite{ronneberger2015u} comprised of transformer and convolutional layers for performing latent diffusion in the latent space $z$, starting from a random Gaussian noise. 
\end{itemize}

By default, LDMs only take text prompts as the input for image generation. In \ourmodel, we extend LDM to condition the image generation on both text (progression description) and an image (prior image). 

to train an image-and-text conditioned diffusion model with the objective function:
\begin{equation}
    \min_{\theta} \mathcal{L} = \mathbb{E}_{z_t, \epsilon \sim \mathcal{N}(0, 1), t}
    \left[||\epsilon - f_{\theta}(z_t, t, \{\textbf{c}_T, \textbf{c}_S\})||_2^2\right]
\end{equation}
where conditions include the textual representations $\textbf{c}_T$ encoded by CLIP~\citep{radford2021learning} text encoder as well as the encoded latent representation $\textbf{c}_S$ for the source image. Following Instruct-Pix2Pix~\citep{brooks2023instructpix2pix}, we concatenate the image condition $\textbf{c}_S$ with $z_t$ and feed them into the LDMs, while using attention layers to cross-attend the text condition $\textbf{c}_T$. The objective is to learn a denoising network $f_{\theta}$ to reconstruct the noise $\epsilon$ given the noisy variant $z_t$ of latent representation for the target image at timestep $t\in \{1,...,T\}$. Once trained, the model can take a source image and textual instruction as inputs to generate a target image. Though the above formula works well for common-domain images~\citep{brooks2023instructpix2pix}, it remains problematic for medical images due to the substantial domain gap. To address this issue and attain a decent model for medical images, we take two further steps.

First, instead of using the CLIP text encoder which was trained on web-crawled image-text pairs, we resort to the text encoder in BiomedCLIP~\citep{zhang2023large}, which is more experienced with biomedical corpus. In this case, the default context length is significantly expanded from 77 up to 256, which can handle more detailed descriptions in clinical reports. To connect the mismatched text encoder and UNet, we introduce a learnable linear project layer in between.
% It turns out that this replacement significantly improves the performance as we will show in our experiments.

Second, we propose a two-stage training strategy. Due to the limited number of paired data, we find training \ourmodel directly leads to considerable overfitting and the model is prone to produce out-of-domain images. The proposed two-stage training strategy can train our \ourmodel model with both unpaired and paired images:
% \chunyl{From the current description, I do not see how \ourmodel is initialized: the language model is BioMedCLIP, and UNet is the weights from InstructP2P? If yes, the two components are not well aligned. If so, Stage-1 also plays of the role of aligning two modalities?}

\begin{itemize}[leftmargin=*]
    \item \textbf{Stage-1: Pre-training.} In this stage, we exploit all images that are with medical reports to learn $f_{\theta}$ in \ourmodel. Instead of using a source image as the condition, we come up with a pseudo source image $I_p = \{128\}^{H \times W \times 3}$ with constant value 128, and encode this into $\textbf{c}_S$, which is then combined with $\textbf{c}_T$ as the paired condition to the LDMs. 
    % \chunyl{the details on how to construct the pseudo source image is missing. If it is random noise, please clarify it.}
    \item \textbf{Stage-2: Instructed Tuning.} After the state-1 pre-training, the model already gets adapted to the medical domain (both images and texts). Without any model modification, we finetune the model with the paired data. The only difference from stage-1 is that we use a real source image $I_s$ rather than a pseudo one $I_p$.
\end{itemize}
\chunyl{Please make sure the notations for images are consistent, it is only bold at the beginning of Section4.1, but not in the rest of the paper, including here and  Section 5.4 in experiments.}

\subsection{Evaluation Metrics}

For evaluation, we assemble a set of instances each comprising two images taken at different times for a given patient, their corresponding reports, and the GPT-4 generated progression description by synthesizing the two reports. 
At test time, \ourmodel inputs the first image and progression description and outputs the counterfactual image. The second image is used as the reference standard for generation.

Ideally, the counterfactual image should accurately reflect the prescribed changes in disease pathology while minimizing deviation from the prior image. 
We propose the Counterfactual Medical Image Generation (CMIG) score that balances accuracy and feature retention measurements. 
Given accuracy measurements $a_1,\cdots,a_n$ and feature retention measurements $f_1,\cdots,f_m$, we first compute their respective geometric means $\bar{a}=\sqrt[n]{\prod_i a_i}$ and  $\bar{f}=\sqrt[m]{\prod_j f_j}$, and then return the CMIG score as their geometric mean $\sqrt{\bar{a}\cdot\bar{f}}$. This ensures that the final score is not skewed to either aspect, as they are both important for counterfactual generation. We choose geometric mean as it is robust to results of varying scales. The CMIG scoring scheme is general. In this paper, we adopt a simple instantiation using a pathology classifier for accuracy, a race classifier and an age classifier for feature retention.

\begin{itemize}[leftmargin=*]
    \item \textbf{Pathology Classifier:} We use the DenseNet-121 model from the XRV collection \cite{cohen2021gifsplanation}, a state-of-the-art image classifier for CheXpert findings~\cite{irvin2019chexpert}. 
    We run it on the counterfactual image to obtain the predicted pathology finding labels. 
    Following RoentGen~\cite{chambon2022roentgen} to enable head-to-head comparison, 
    we run CheXpert~\cite{irvin2019chexpert} on the corresponding report of the reference image to obtain reference pathology labels, focusing on the five most prevalent findings (Atelectasis, Cardiomegaly, Edema, Pleural Effusion, Pneumothorax), and then 
    compute AUROC of the predicted labels against the reference ones. 
    %Specifically trained on genuine images from the p19 test set and 1,214 generated images, this model discerns essential pathological characteristics. The images underwent a series of processing steps: resizing to 512 px, center cropping, and adjusting to a resolution of 224 x 224 px, ensuring compatibility with the model's requirements. Labels derived from associated reports through NLP acted as the reference standard.        \item \textit{Metric:} The primary evaluation metric was the AUC, placing particular emphasis on the average AUC for conditions like Atelectasis, Cardiomegaly, Edema, Pleural Effusion, and Pneumothorax, following \cite{chambon2022roentgen}.    
    
    \item \textbf{Race Classifier:} Similarly, we use the state-of-the-art image classifier for race~\cite{Gichoya2022} to generate predicted labels on the system-generated counterfactual images, gold race information from MIMIC as reference labels, and compute AUROC.
    %The importance of accurately identifying race from medical images—using the gold standard data from MIMIC-IV—cannot be understated given its potential clinical implications \cite{Gichoya2022}. \item \textit{Metric:} The AUC served as the primary evaluation metric.    
    
    \item \textbf{Age Classifier:} We use the state-of-the-art DNN model~\cite{Ieki2022} to predict age from the image, the anchor age information from MIMIC as reference, and return Pearson correlation. MIMIC only contains patient data within a short duration, so the two images are taken when the patient is approximately at the anchor age.
    
    %Leveraging a pretrained DNN model \cite{Ieki2022}, we sought to measure the correlation between predicted and actual ages using data from the MIMIC-IV dataset. The relevance of accurately predicting age in a clinical context is accentuated by \cite{Ieki2022}.   \item \textit{Metric:} The Pearson correlation coefficient was employed to compare predicted and actual ages.
    
\end{itemize}

    
%     \item \textbf{Segmentation Model:} We incorporated a pretrained chest x-ray segmentation model, which amalgamates anatomical structure, contextual cues, and disease relations \cite{Lian2021}.
%     \begin{itemize}
%         \item \textit{Metric:} Dice Score between the predicted and actual image segmentations.
%     \end{itemize}
% \end{itemize}

% \subsubsection{Calculation of the \ourmodel{} Score}

% The \textit{\ourmodel{} Score} acts as an integrated metric, synergizing the AUC score derived from pathology classification, represented as \(S_{\text{path}}\), and the geometric average of three patient feature preservation scores, denoted as \(A_{\text{feat}}\). The formal definition using the geometric average for both components is:

% \begin{equation}
% \text{\ourmodel{} Score} = \sqrt{S_{\text{path}} \times A_{\text{feat}}}
% \end{equation}

% with

% \begin{align*}
% A_{\text{feat}} = \sqrt[3]{\text{Age Pearson Correlation} \times \text{Race AUC} \times \text{Segmentation Dice}}
% \end{align*}

% The choice of the geometric mean ensures that each metric contributes equitably to the overall \ourmodel{} Score. This approach emphasizes the combined importance of clinical relevance and feature preservation for a comprehensive evaluation. The \ourmodel{} Score provides a unified measure, encapsulating both diagnostic precision and the fidelity of patient-specific features in the generated images.




